Strawberry Fields: A Software Platform for Photonic Quantum Computing

We introduce Strawberry Fields, an open-source quantum programming architecture for light-based quantum computers, and detail its key features. Built in Python, Strawberry Fields is a full-stack library for design, simulation, optimization, and quantum machine learning of continuous-variable circuits. The platform consists of three main components: (i) an API for quantum programming based on an easy-to-use language named Blackbird; (ii) a suite of three virtual quantum computer backends, built in NumPy and TensorFlow, each targeting specialized uses; and (iii) an engine which can compile Blackbird programs on various backends, including the three built-in simulators, and -- in the near future -- photonic quantum information processors. The library also contains examples of several paradigmatic algorithms, including teleportation, (Gaussian) boson sampling, instantaneous quantum polynomial, Hamiltonian simulation, and variational quantum circuit optimization.

==> diagrams/gate_teleportation_circuit.tex <==
\Qcircuit @C=1em @R=1em {
     \lstick{q_0:~\ket{\psi}~~} & \ctrl{1}  & \qw & \gate{F^\dagger} & \meter & \rstick{\hspace{-0.2cm}\ket{x}\bra{x}=m_1}\\
     \lstick{q_1:P\ket{0}_P} & \ctrl{0}  & \ctrl{1}& \gate{F^\dagger} & \meter & \rstick{\hspace{-0.2cm}\ket{x}\bra{x}=m_2}\\
     \lstick{q_2:~\ket{0}_P~} & \qw & \ctrl{0} &\qw & \qw &\qw &\rstick{\hspace{-0.2cm}X(m_2)FPX(m_1)F\ket{\psi}}
}

